Modelling Compositionality and Structure Dependence in Natural Language

Human beings possess the most sophisticated computational machinery in the known universe. We can understand language of rich descriptive power, and communicate in the same environment with astonishing clarity. Two of the many contributors to the interest in natural language - the properties of Compositionality and Structure Dependence, are well documented, and offer a vast space to ask interesting modelling questions. The first step to begin answering these questions is to ground verbal theory in formal terms. Drawing on linguistics and set theory, a formalisation of these ideas is presented in the first half of this thesis. We see how cognitive systems that process language need to have certain functional constraints, viz. time based, incremental operations that rely on a structurally defined domain. The observations that result from analysing this formal setup are examined as part of a modelling exercise. Using the advances of word embedding techniques, a model of relational learning is simulated with a custom dataset to demonstrate how a time based role-filler binding mechanism satisfies some of the constraints described in the first section. The model's ability to map structure, along with its symbolic-connectionist architecture makes for a cognitively plausible implementation. The formalisation and simulation are together an attempt to recognise the constraints imposed by linguistic theory, and explore the opportunities presented by a cognitive model of relation learning to realise these constraints.

==> chapters/Results.tex <==



==> chapters/notes_on_comments.tex <==
1. Added the notch to make it clear that it is only a pushout in fig 2.1. 
2. Word orders vary across languages, and accordingly, Merge results in different deep structures for different languages. To illustrate why they are different, Kannada is a good example.
3. A big part of the formalisation is trying to connect what is known about compositionality, to what is known about how DORA processes information. So if some of the functions do not seem to make sense at first, they will become clear when DORA's functioning is discussed. 
4. Some of the linguistic ideas are hard to grasp, but I am afraid it is very hard to get into the finer details, given the limit on thesis length. And so I have included standard reference papers in the bibliography.



==> chapters/random.tex <==
In \cite{pagin_compositionality_2010}, the authors consider \texit{synonymy} to be the basis for the equivalence relation. That is, for a constituent to be substituted, it must have identical meaning. To perform a broader and independent analysis, we instead treat the equivalence relation as a time pattern of lexical projections to keep idea of grammar as distinct. 

DORA is capable of modelling all three versions of the weak complexity - It currently uses coactivation of P's alone to map. It is possible to form recursive definitions of this to include compositional mapping.

Relational thinking implicitly assumes the presence of an object and the role played by the object. Human beings have no trouble distinguishing between the phrases - `big house' and `big tractor', automatically assuming that the house and tractor are qualified by the property of bigness. \\

This relates neatly to the property of natural language propositions and the Binary Branching Hypothesis [..cite antisymmetry..] that treats every complete proposition as a binary tree, where each node can dominate at most two nodes. 


I was quite unsure at the start of my Master's degree about my field of specialisation. As a result of many happy coincidences and the freedom TUM affords its students, I was able to study machine intelligence and computational neuroscience, before finally settling on the optimum plane of Computational Cognitive Modelling. I would like to thank Dr. Andrea E Martin for introducing me to this fascinating area and being an ever supportive mentor.

I thank Dr. Christina Kuttler for taking on the role of examiner at such a short notice. Her supportive emails have kept me calm throughout my thesis. Dr. Bernhard Werner helped me iron out my ideas, and structure this thesis. I thank him.

I also thank Cas Coopmans, who helped start this project by giving me helpful tips and pointing me to resources in linguistics.

My friends have provided entertainment, cooked for me, and reviewed my thesis (not necessarily in that order) when I needed it most. I thank them, and my parents, who have been a constant source of emotional support.

\subsection{Action planning and action grammar}

To contrast the grammar and structure dependence found in language, we look at another human capacity - that for complex action planning. It has been suggested [..] that the syntax of language and music is a descendent of the more basic sequential action system. A purely sequential, non compositional system is not capable of explaining the persistence of goals and sub-goals in a complex action setup. 
Although this has received a lot of attention conceptually, the theoretical reasons for the differences between language and action planning have not been made clear, and I attempt to do just that in this section.\\ 

We consider the coffee making example from [...] as shown in figure \ref{coffee-making}. Following the formalisation setup in the preceding sections, we define the $L_{0}$ as the set of atomic actions - \{ Fill water, Grind coffee, Machine makes coffee, Put coffee in machine, Take container, Turn on machine\}. In order to lend significance to the idea of a syntax in action planning, the constituents are assigned labels in [...] ie., Prep and Head, analogous to NP,VP etc., This is a matter of debate, as there is no principled way to define what or where these labels come from, and may also hold clues as to what we consider grammar in the first place. But there is a more fundamentally disturbing issue with assigning such labels. Consider switching the position of the $L_{2}$ `Head', to the left. Not only does the constituent lose meaning, it also becomes physically impossible to expect the machine to make coffee. In language on the other hand, constituent meaning itself cannot be destroyed based on position alone. \\

Let us for the time being assume that this kind of labelling is fair and sensible. Also, the idea of a constituent itself can be defended by considering the ability to be substituted by one action to be a necessary condition for anything to be called a constituent. For example, in the example shown - ``Take container and fill water" can be replaced by ``Supply water". Based on the figure \ref{StoT}, we can then safely assume that every \textbf{physically possible} set of action sequences can be decomposed into their $L_{i}$s.

\subsubsection{No more a partial function}
The equivalent of \mathbb{H} in action planning can be taken to be \mathbb{G} where G is the set of goals that a given agent can perform. Given a sequence of actions $s\in S$, we can define $g:s\to{T,F}$ where $g$ relates $s$ to the boolean value of the action it completes. 
Any structure that we choose to impose on this sequence of actions is completely determinable from the linear order of the sequence itself. 

The human brain is the most complex computing device in the known universe. Of the many dazzling feats a human being is capable of achieving, comprehending natural language occupies a unique place. Therefore, one of the goals of Cognitive Science is understanding what it means to have knowledge of human language. Such a goal also amounts to having the ability to replicate this knowledge, for which computational understanding is key. Compositionality and structure dependence are two essential properties of natural language. Drawing on formal linguistics and set theory, I work on formalising these ideas in the first half of the thesis. 

. The emphasis is on developing a system which is motivated by cognitive processing constraints, including information carried over time. 

I characterise a system capable of satisfying these properties, while keeping with processing constraints, and what we know from neuroscience. I then implement 

----




\subsubsection{Structure dependent operations}
If one considers the case of displacing or moving an existing constituent in order to accomplish another sub-task, knowledge of the organising principle is important. But since we have shown that the arrows going from $S\to T^{*}_{i}$ and $T^{*}_{i}\to \mathbb{G}$ are full functions, it leads to the 

\begin{figure}
\centering
\includegraphics[scale=0.7]{images/coffee_making.pdf}
\caption{Hierarchically organised coffee making}
\label{coffee-making}
\end{figure}

The nature of the set $\mathbb{H}$ and its creation is a subject of debate among linguists. The binary branching requirement is grounded in the minimalist requirement, and is referred to as the Binary Branching Hypothesis or BBH, and is based on the assumption that any non terminal node can dominate at most two daughters. This is based further on the idea of ``unambiguous path" between antecedent and anaphor (That which relates the interpretation of a second expression, anaphor, to the primary expression, antecedent. Ex - I like Fred, he's a middle aged cat (Fred is the antecedent and `he's' the anaphor)). 


- TO DISCUSSION - HOW DORA MAPS ONTO FORMALISATION
- ACTIVATION PATTERNS -
- 
- WHY RNNs DON'T CUT IT
- GRAMMAR INDUCTION
- TOP DOWN in perception, BOTTOM UP in inference

An example of a system that has compositionality is illustrated by constructions involving lego blocks. If one were to construct a toy house with these blocks, compositionally, it would be straightforward enough to combine similar shapes into a roof, walls, door etc., while still maintaining the structural integrity of every individual block. But nothing definite can be said about recursion in this setup. 

To give an example from a completely different domain - Picture groups of people banding together, starting from the smallest unit, a family, and combining to form larger and larger groups of people, each having one or many representatives, with progressively increasing responsibilities. How does this relate to language, one might ask.





###### Definitions 

Semantic layer - Common to all PO units, where every unit represents a single dimension along which predicate/object is encoded.

Link weights - Connect PO units to the semantic layer. Activations are passed as a factor of link weight.

PO Layer - Unit represents individual predicates and objects. Objects can contain higher order propositions.

RB layer - Unit represents the binding of role (predicate) and filler (object).

P layer - Unit represents the overall proposition

Local inhibitor - Every unit (except unit in semantic layer) is coupled with an inhibitor. Once the activation of the unit it is coupled with goes over the threshold $\phi_{L}$, the local inhibitor resets the activation of the unit to zero, by setting its own activation to $\tau_{L}$.

Global inhibitor - Acts as a global refresh signal, which resets all unit activations to zero (by setting its own activation to $\tau_{G}$) if any RB unit activation is greater than $\phi_{G}$. 

Analog - All propositions belonging to a single story/environment, which reuse objects and predicates amongst their propositions. 

Driver - Represents the Field of Attention of DORA. All activations start in the Driver, and flow into the Recipient or LTM.

Recipient - Contains the propositions which are retrieved from LTM to enable mapping.

Long term memory (LTM) - Contains all the propositions from all analogs.

Phase set - Set of mutually desynchronised role-filler bindings


\begin{enumerate}
    \item\label{s1} Initialise driver with a set of propositions.
    \item\label{s2} Set all activations to zero
    \item\label{s3} Set firing order of POs (currently set to the order of arrangement within each proposition)
    \item\label{s4} Run the following operation three times (=1 phase set). Update the activations until the local inhibitor fires
    \begin{enumerate}[label*=\arabic*.]
        \item\label{s4.1} Updates modes of P units
        \item\label{s4.2} Update inputs to all token units in Driver
        \item\label{s4.3} Update input to semantic layer
        \item\label{s4.4} Update input to all units in the Recipient
        \item\label{s4.5} Update activations of all units
        \item\label{s4.6} Run retrieval routine (if Recipient is empty)
        \item\label{s4.7} Update all mapping hypotheses (if Recipient is not empty)
    \end{enumerate}
    \item Update mapping connections
\end{enumerate}


\begin{longtable}{|p{2cm}|p{\linewidth-3cm}|}
\hline
Term & Description \\[0.5ex] 
\hline\hline
Merge & It is a binary operation on two syntactic objects X,Y to construct a third object Z, which is simply the set X\cup Y. \\
Syntactic projection (as used here) & The lexical label given to a word\\
Deep Structure &  The underlying logical relationships of the elements of a phrase or sentence\\
Externalisation & - the mapping from internal linguistic representations to their ordered output form, either spoken or manually gestured \\
Move & The transformation on deep structure which rearranges word order for externalisation\\
Wh-movement & Is a phenomenon where the interrogative word (Who, what etc.) appears at a different position from the answer.\\
Head & Within a constituent,there is usually a single element which is of primary importance in determining the grammatical behavior of the whole unit. Such a word or phrase is called the head. Ex - In ``The temples of India'', the word ``temples'' determines the agreement on the verb which comes after the phrase, and is therefore the head\\
Xbar theory & A structural setup for defining a phrase, which contains a head. The main idea behind the development of this theory is that all phrase structure can be reduced to simple recursive operations on basic configurations containing the head\\
Complement & The phrasal constituent which is the sister (Two sister constituents are inputs to a Merge operation) of a head\\
Specifier &  The phrasal constituent which is the sister of the mother (the product of Merge operation on two sisters) of the head\\
\hline
\end{longtable}


null hyp - word embedding does not affect precision
alt hyp - word embedding does affect it



==> components/acknowledgements.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Acknowledgements}

\vspace*{2cm}

\begin{center}
{\Large \textbf{Acknowledgments}}
\end{center}

I was quite unsure at the start of my Master's degree about my field of specialisation. As a result of many happy coincidences and the freedom TUM affords its students, I was able to study machine intelligence and computational neuroscience, before finally settling on Computational Cognitive Modelling and linguistics. I thank Dr. Andrea E Martin for introducing me to this fascinating area, taking an active interest in this project, and being an ever supportive mentor.\\

Dr. Bernhard Werner helped me structure this thesis, and made me realise the importance of keeping text reader friendly, which I have attempted to do, to the best of my abilities. I thank him. I thank Dr. Christina Kuttler for taking on the role of examiner at short notice. Her quick and kind emails have kept me calm throughout.\\

I also thank Cas Coopmans, who helped start this project by giving me helpful tips and pointing me to resources in linguistics. My friends have provided entertainment, cooked for me, and reviewed my thesis (not necessarily in that order) when I needed it most. I thank them, and my parents, who have been a constant source of emotional support.



==> components/cover.tex <==
% !TEX root = ../main.tex
% The front cover.
% Included by MAIN.TEX

%--------------------------------------------------
% The Front Cover
%--------------------------------------------------

% correct BCOR - undo at the end !!!
\def\bcorcor{0.15cm}
\addtolength{\hoffset}{\bcorcor}

\thispagestyle{empty}

\vspace{4cm}
\begin{center}
	\includegraphics[width=4cm]{\universityLogo}\\
	\vspace{5mm}
	\huge \program \\
	\vspace{0.5cm}
	\large \university
\end{center}

\vspace{20mm}
\begin{center}
	{\Large \doctype}\\
	\vspace{20mm}
	{\huge \textbf \title}\\
	\vspace{15mm}
	{\LARGE  \author}\\
	\vspace{\fill}
	\includegraphics[width=4cm]{\programLogo}
\end{center}


==> components/disclaimer.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage

\thispagestyle{empty}
\vspace*{0.8\textheight}
\noindent
I hereby declare that this thesis is entirely the result of my own work except where otherwise indicated. I have only used the resources given in the list of references.

\vspace{15mm}
\noindent
\date \hspace{5cm} \author
\newpage


==> components/outline.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage

\phantomsection
\addcontentsline{toc}{chapter}{Outline of the Thesis}

\begin{center}
	\huge{Outline of the Thesis}
\end{center}


%--------------------------------------------------------------------
\section*{Part I: Introduction and Theory}

\noindent {\scshape Chapter 1: Introduction}  \vspace{1mm}

\noindent  This chapter presents an overview of the thesis and it purpose. Furthermore, it will discuss the sense of life in a very general approach.  

\noindent {\scshape Chapter 2: Theory}  \vspace{1mm}

\noindent  No thesis without theory.   \vspace{1mm}

%--------------------------------------------------------------------
\section*{Part II: The Real Work}

\noindent {\scshape Chapter 3: Overview}  \vspace{1mm}

\noindent  This chapter presents the requirements for the process.
%--------------------------------------------------------------------
\section*{Part III: Future Work}

\noindent {\scshape Chapter 3: Overview}  \vspace{1mm}

\noindent  This chapter presents the requirements for the process.


==> components/preface.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Preface}	


\vspace*{3cm}

\begin{flushleft}
{\Large \bf Preface}
\end{flushleft}

\vspace{1cm}




\newpage

==> components/quote.tex <==
\clearpage
\phantomsection

\begin{center}
\vspace*{11cm}
\textit{``Everything should be made as simple as possible, but not simpler''}
\end{center}
\par
\hspace*{7cm}
\textit{-Albert Einstein}


==> components/titlepage.tex <==
% !TEX root = ../main.tex
% The titlepage.
% Included by MAIN.TEX


%--------------------------------------------------
% The title page
%--------------------------------------------------

% correct BCOR - undo at the end !!!
\def\bcorcor{0.15cm}
\addtolength{\hoffset}{\bcorcor}

\thispagestyle{empty}

\vspace{4cm}
\begin{center}
    \includegraphics[width=4cm]{\universityLogo}\\
    \vspace{5mm}
    \huge \program \\
    \vspace{0.5cm}
    \large \university
\end{center}

\vspace{10mm}
\begin{center}
    {\Large \doctype}\\
    \vspace{10mm}
    {\LARGE \title}\\
    \vspace{10mm}

    \begin{tabular}{ll}
      \Large Author:                        & \Large \author \\[2mm]
      \Large Examiner:& \Large \examinerOne\\[2mm]
      \Large Advisor:& \Large \Advisorone \\[2mm]
      \Large Advisor:& \Large \Advisortwo \\[2mm]
      \Large Submission Date:& \Large \date
    \end{tabular}

    \vspace{\fill}
    \includegraphics[width=4cm]{\programLogo}
\end{center}

% undo BCOR correction
\addtolength{\hoffset}{\bcorcor}


==> main_orig.tex <==
% Important: The shell-escape flag is required for the Minted package.
% Please compile this document with 'pdflatex -shell-escape main.tex'.
% If you are using another IDE, you may be able to specify this in the
% options or to provide an option like '% !TEX option = -shell-escape'
% in this file, depending on your builder. See the README.md for more.

% Don't put any content in here.
% Don't even include content files by using \input or \inlcude.
% Put your content into components/text.tex or include it there using \input.
% You probably want to modify the following files:
%   components/info.tex             contains the author, title etc.
%   components/settings.tex         contains the packages and settings.
%   components/commands.tex         contains helpful custom commands.
%   components/glossary.tex         contains an explanation of the used terms.
%   components/acknowledgements.tex contains the acknowledgements.
%   components/quote.tex            contains a quote.
%   components/abstract.tex         contains the abstract of the document.
%   components/text.tex             includes the actual content of the document.
%   components/outline.tex          contains the outline.
%   components/preface.tex          contains the preface.
%   chapters/                       contains the main text.
%   bibliography/literature.bib     contains the BibTeX entries.
%   images/                         contains all your content-related images.
%
% You probably don't need to change anything in the following files:
%   components/cover.tex            formats the front cover of the document.
%   components/titlepage.tex        formats the title page of the document.
%   components/disclaimer.tex       formats the disclaimer page.
%   styles/                         contains style elements (e.g. logos).
%   main.tex                        contains the top-level code structure.
%   README.md                       contains information about this template.

%\documentclass[11pt,
%              a4paper,
%              index=totoc,
%              headsepline,
%              footsepline,
%              BCOR=12mm,
%              DIV=13]{scrbook}

% KOMA scrbook options:
%  index=totoc: include an entry for the index in the table of contents.
%  headsepline: use horizontal line under heading.
%  footsepline: use horizontal line above footer.
%  BCOR: binding correction (e.g.: BCOR=12mm)
%  DIV: Number of sheet sections (used for layout) (e.g.: DIV=13)


%  This code base is currently hosted at: 
%  https://github.com/waltsims/TUM_Thesis_Template_CSE
             
\input{components/info}

\input{components/settings}

\input{components/commands}

\input{components/glossary}

\makeglossaries

\begin{document}

 \frontmatter

 \input{components/cover}

 \clearemptydoublepage

 \input{components/titlepage}

 \input{components/disclaimer}

 \input{components/acknowledgements}

 %\input{components/quote}

 \input{components/abstract}

 \tableofcontents

 \mainmatter

 \input{components/text}

 \clearemptydoublepage

 \printglossaries

 \addcontentsline{toc}{chapter}{Bibliography}
 \bibliography{bibliography/export-data.bib}

\end{document}

